Learning to Remember: Advances in Memory Mechanisms for Large Language Models

Memory has become a central mechanism for extending large language models (LLMs) beyond fixed context windows, stateless interaction, and static parametric knowledge. This survey organizes the literature around three complementary dimensions: the life cycle of memory, the storage substrate, and the system role that memory plays in LLM-based agents, while using cognitive-science-inspired memory concepts as a lightweight conceptual motivation rather than as a separate technical contribution or implementation family. On this basis, we distinguish three mechanism families: nonparametric memory, where information is stored outside model parameters in text, graph, multimodal, or database-like structures; parametric memory, where information is stored or accessed through activations, key-value caches, learned modules, adapter-based parameterizations, or model weights; and memory for agent evolution, where stored experiences support reinforcement learning, continual learning, procedural reuse, context engineering, and agent harness design. Evaluation is treated as a separate cross-cutting component rather than as a memory mechanism. Unlike surveys that focus primarily on retrieval-augmented generation or long-context modeling, this paper emphasizes the full memory life cycle: construction, maintenance, retrieval, consolidation, forgetting, governance, and evaluation. By aligning conceptual motivations, computational memory mechanisms, benchmarks, and deployment concerns, the survey provides a structured roadmap for designing memory-augmented LLM agents that are persistent, adaptive, auditable, and safe to update over time.

==> section/benchmark.tex <==
Evaluating the effectiveness of memory-augmented large language models (LLMs) requires rigorous benchmarking to assess their ability to retain, recall, and reason across extended contexts. While architectural innovations provide the mechanisms for storing and managing information, benchmarks reveal whether these mechanisms translate into meaningful performance gains in practice. Current evaluation efforts encompass both text-only and multimodal settings, ranging from controlled synthetic tasks that probe retrieval precision to complex, multi-session, real-world scenarios demanding long-horizon reasoning and adaptation. This section surveys the major benchmarks developed for memory in LLMs, categorizing them into text-based evaluations and multimodal datasets, and highlighting how they test different aspects of memory such as persistence, coherence, and contextual integration.

\subsection{Text-only Benchmarks}
A large body of benchmarks for evaluating memory in LLMs rely on text-only settings, focusing on whether models can retain, recall, and reason over information across extended contexts. These benchmarks vary in scope, from controlled synthetic retrieval tasks to complex, real-world scenarios that demand persistent reasoning across multiple sessions.

\subsubsection{Basic Capabilities}
Basic benchmarks focused on controlled, text-only settings to probe whether LLMs could retain and utilize information across extended contexts. These benchmarks typically emphasize retrieval, recall, and short-term reasoning.

Needle in a Haystack serves as a focused test of in-context retrieval ability within long contexts.
The benchmark places a random fact or statement (the 'needle') in varying positions within extended contexts (the 'haystack'),
then measures the model's precision in retrieving this information.
Through systematic variation of document depths and context lengths, it provides quantitative assessment of retrieval performance.
%https://github.com/gkamradt/LLMTest_NeedleInAHaystack?tab=readme-ov-file

$\infty$Bench~\citep{zhang2024inftybenchextendinglongcontext} pushes the evaluation frontier to contexts exceeding 100K tokens, with an average input length of around 200K.
It introduces both synthetic and realistic tasks across retrieval, code, math, novels, and dialogue. The synthetic retrieval tasks (such as passkey lookup, digit sequence extraction, or key–value mapping) assess whether models can locate fine-grained information in extremely long contexts, while more realistic tasks based on novels and dialogue probe reasoning and summarization abilities. Importantly, $\infty$Bench demonstrates that even state-of-the-art long-context models exhibit significant degradation when context length is scaled to hundreds of thousands of tokens.

LongMemEval~\citep{wu2025longmemevalbenchmarkingchatassistants} focuses specifically on long-term interactive memory by proposing 500 curated questions embedded within extended user–assistant chat histories. It defines five core memory abilities—information extraction, multi-session reasoning, temporal reasoning, knowledge updates, and abstention—making it one of the first benchmarks to systematically probe memory-related skills beyond simple retrieval. By emphasizing the interactive nature of assistant-style conversations, it highlights how memory is required not only for fact recall but also for maintaining consistency and adapting to evolving user information.

OdysseyBench~\citep{wang2025odysseybenchevaluatingllmagents} introduces a benchmark for long-horizon workflows in productivity tasks, including Word, Excel, PDF, Email, and Calendar. Unlike earlier retrieval-oriented benchmarks, OdysseyBench requires agents to track context across multiple steps, integrate information from prior exchanges, and coordinate actions across different applications. With both real-world–inspired tasks and synthetically generated ones, it situates memory evaluation in the context of practical office assistant scenarios.

LOCOMO~\citep{maharana2024evaluatinglongtermconversationalmemory} shifts the focus to very long-term conversational memory, collecting dialogues that span up to 35 sessions and around 9K tokens per conversation. Its benchmark tasks—question answering, event summarization, and dialogue consistency—explicitly test whether models can sustain long-range causal and temporal coherence. This design mirrors real-world conversational agents that must remember user personas, events, and preferences across extended time horizons.

LongBench~\citep{bai2024longbenchbilingualmultitaskbenchmark} was one of the first multitask bilingual benchmarks explicitly designed for long-context evaluation. It covers 21 datasets across six categories, including single- and multi-document question answering, summarization, few-shot learning, code completion, and synthetic retrieval tasks. By standardizing diverse tasks into a unified format and reporting results with automatic metrics (e.g., F1, ROUGE, accuracy), LongBench provides a foundation for systematically comparing LLMs’ ability to process texts much longer than their standard training contexts.
In addition, LongBench v2~\citep{bai2025longbenchv2deeperunderstanding} extends the long-context evaluation landscape even further, both in length (up to 2M words) and in task diversity. It includes single- and multi-document QA, long in-context learning, long dialogue history understanding, code repository comprehension, and structured data reasoning. Unlike earlier benchmarks where many tasks could still be solved by shallow retrieval, LongBench v2 explicitly designs questions that demand deep reasoning and multi-step integration, making it a more challenging testbed for evaluating whether models can truly comprehend and synthesize information across vast contexts.

\subsubsection{Comprehensive Capabilities}
In contrast, comprehensive benchmarks aim to evaluate the end-to-end memory proficiency of LLMs across complex, realistic, and often multi-session settings. They integrate reasoning, temporal and causal understanding, and context synthesis into the evaluation, going beyond isolated retrieval.

StoryBench 
~\citep{NEURIPS2023_f63f5fbe}
introduces a dynamic evaluation paradigm focused on interactive narrative reasoning.
Diverging from synthetic tests (e.g., Needle-in-a-Haystack) or conventional dialogue evaluations,
StoryBench simulates real-world memory demands through branching storylines where decisions propagate consequences.
The benchmark's innovative framework comprises 311 interconnected scenes with 86 decision points,
testing both knowledge retention (turn-to-turn coherence) and sequential reasoning (causal decision tracking).
StoryBench further innovates through dual evaluation modes:
Immediate feedback (assessing short-term error correction) and
self-recovery (evaluating autonomous mistake revision capabilities).

Minerva 
~\citep{xia2025minervaprogrammablememorytest}
contributes a unique programmable framework for decomposing memory capabilities into fundamental operations.
Unlike holistic benchmarks, Minerva enables precise examination of core memory functions through:
Atomic tests evaluating isolated skills (search, recall, edit, and stateful processing), and
composite tests simulating real-world scenarios through task combinations.
This modular approach facilitates the targeted analysis of specific memory subsystems and their interactions.


\subsection{Multimodal Benchmarks}
The rapid development of multimodal large language models has highlighted the need for benchmarks that go beyond short clips and test systems on long-form, temporally complex video understanding. Unlike text-only evaluations, multimodal benchmarks must capture the interplay between visual and linguistic information across extended time spans, where memory, temporal reasoning, and narrative comprehension are critical. Recent datasets have pushed the field forward by curating long videos, diverse question types, and evaluation protocols that expose the limitations of current models. 

MovieQA~\citep{Tapaswi_2016_CVPR} is one of the first large-scale benchmarks for narrative video understanding, with 14,944 multiple-choice QAs over 408 movies. It integrates five modalities—video clips, plots, scripts, subtitles, and DVS—to test both visual and textual reasoning. Around 6,462 QAs are time-aligned with clips, enabling multimodal evaluation. While influential, MovieQA remains limited in temporal scope compared to newer long-form datasets.

MoVQA~\citep{zhang2023movqabenchmarkversatilequestionanswering} is a dataset of 21,953 QA pairs from 100 movies spanning single-scene, multi-scene, and full-movie contexts. Questions are grouped into six types including synopsis, causal and hypothetical reasoning, and external knowledge. Unlike earlier movie datasets, MoVQA explicitly considers both clue length and video length to evaluate temporal difficulty. Results show clear performance drops as temporal scales increase, underscoring memory challenges in multimodal QA.

MovieChat+~\citep{song2024moviechatquestionawaresparsememory} is a system and benchmark for ultra-long videos (>10K frames). Inspired by human memory models, it introduces a question-aware sparse memory that consolidates tokens based on relevance, reducing redundancy while preserving context. The accompanying MovieChat-1K benchmark provides 1K long videos, 14K QA pairs, and 2K temporal labels. MovieChat+ outperforms prior video-language models and remains efficient in handling both long and short video QA.

EgoSchema~\citep{NEURIPS2023_90ce332a} is a diagnostic benchmark of 5,063 QAs over 250 hours of egocentric video. Each question is tied to a three-minute clip, making it substantially longer than typical QA datasets. It introduces temporal certificates to quantify the intrinsic reasoning length, with a median of 100 seconds—far exceeding other datasets. Evaluations show state-of-the-art models below 33\% accuracy versus 76\% for humans, highlighting the difficulty of very long-term multimodal reasoning.

CinePile~\citep{rawal2024cinepilelongvideoquestion} is a large-scale dataset of 305,000 questions from nearly 9,400 movie clips. Built using audio descriptions and LLM-driven generation with human refinement, it spans temporal, narrative, thematic, and perceptual reasoning. CinePile’s adversarial filtering ensures non-trivial questions, making it both a training resource and a rigorous evaluation set, where current MLLMs still lag far behind human performance.

LongVideoBench~\citep{NEURIPS2024_329ad516} is a benchmark for hour-long subtitled videos with 6,678 human-annotated multiple-choice questions. It introduces referring reasoning, where questions reference specific video contexts to test fine-grained perception and relational reasoning. Covering 17 categories, it mitigates single-frame bias and shows that even advanced LMMs like GPT-4o struggle with long-term reasoning, while performance improves only when more frames are processed.

LVBench~\citep{wang2025lvbenchextremelongvideo} is a benchmark for evaluating MLLMs on long-form videos averaging over an hour. It defines six core skills—temporal grounding, summarization, reasoning, entity recognition, event understanding, and information retrieval—to test models’ memory and reasoning over extended contexts. With carefully curated human annotations, LVBench highlights the persistent difficulty of sustaining coherent understanding across thousands of frames.

Video-MME~\citep{Fu_2025_CVPR} covers 900 videos across six domains and thirty categories. Unlike prior datasets, it integrates subtitles and audio alongside video frames, enabling a broad test of multimodal memory. Results show that additional modalities significantly boost performance, especially for longer videos, while revealing a large gap between commercial and open-source models.


==> section/benchmark_legacy.tex <==

% TO BE REVISED
Evaluating the memory capabilities of large language models (LLMs) requires carefully
designed benchmarks that assess both basic retrieval and complex, long-term reasoning. 
Existing benchmarks vary significantly in scope, methodology, and evaluation focus—ranging 
from controlled synthetic tasks to dynamic, real-world simulations. 
This section systematically reviews prominent benchmarks, 
categorizing them into those measuring fundamental retrieval abilities (Basics) 
and those testing higher-order memory functions (Comprehensive Capabilities). 
By analyzing their distinct designs—including context length, task diversity, 
and evaluation metrics—we highlight how each contributes to understanding LLM 
memory limitations and advancements.

\subsection{Basics}

Needle in a Haystack
serves as a focused test of in-context retrieval ability within long contexts.
The benchmark places a random fact or statement (the 'needle') in varying positions within extended contexts (the 'haystack'),
then measures the model's precision in retrieving this information.
Through systematic variation of document depths and context lengths, it provides quantitative assessment of retrieval performance.
%https://github.com/gkamradt/LLMTest_NeedleInAHaystack?tab=readme-ov-file

In contrast, LoCoMo (Long-Term Conversational Memory)
~\citep{maharana2024evaluatinglongtermconversationalmemory}
adopts a more holistic approach by evaluating three distinct capabilities: question answering across diverse query types (single/multi-hop, temporal, and adversarial),
event summarization requiring extraction of causal/temporal relationships, and
multi-modal dialogue generation demanding persona-consistent responses incorporating images.
The benchmark comprises 50 extensive dialogues (averaging 300 turns and 9K tokens across up to 35 sessions),
constructed through LLM-generated interactions grounded in detailed personas and temporal event graphs,
subsequently refined by human annotators for consistency.
LoCoMo's distinctive value lies in its emphasis on longitudinal conversational dynamics,
offering a framework for developing memory-aware, contextually grounded dialogue systems.

LongMemEval
~\citep{wu2025longmemevalbenchmarkingchatassistants}
extends the evaluation scope further by incorporating five critical dimensions:
information extraction, multi-session reasoning, temporal reasoning, knowledge updates, and abstention capability.
The benchmark features 500 manually curated questions embedded within scalable chat histories
that can extend up to 1.5 million tokens, presenting exceptional scalability challenges.
LongMemEval's systematic categorization includes seven question types:
Single-session-user and single-session-assistant test memorization of user/assistant information within individual sessions.
Single-session-preference evaluates personalized response generation based on user information.
Multi-session (MR) assesses information aggregation across multiple sessions.
Knowledge-update (KU) focuses on tracking changes in user states.
Temporal-reasoning (TR) examines reasoning with both metadata timestamps and explicit time references.
Additionally, modified "false premise" questions (ABS) test the model's ability to appropriately abstain from answering.

%https://arxiv.org/pdf/2410.10813

LongBench
~\citep{bai2024longbenchbilingualmultitaskbenchmark}
establishes itself as a bilingual, multi-task benchmark for comprehensive long-context evaluation,
incorporating 21 datasets across 6 task categories in English and Chinese,
with average lengths of 6,711 words (English) and 13,386 characters (Chinese).
The benchmark spans key application domains including single-doc QA, multi-doc QA, summarization,
few-shot learning, synthetic tasks, and code completion.

LongBench v2
~\citep{bai2025longbenchv2deeperunderstanding}
advances this framework by focusing on deep understanding and reasoning across real-world scenarios.
The updated version contains 503 challenging multiple-choice questions with contexts ranging from 8k to 2M words,
organized into six categories: single-document QA, multi-document QA, long in-context learning,
long-dialogue history understanding, code repository understanding, and long structured data understanding.
The dataset's practical relevance is ensured through contributions from nearly 100 highly educated professionals
representing diverse domains.

Letta
~\citep{packer2024memgptllmsoperatingsystems}
adopts a distinctive architectural perspective by evaluating two fundamental memory systems:
core memory (in-context memory) and archival memory (external memory management).
The benchmark specifically measures stateful agents' capabilities in memory operations:
reading, writing, and updating both memory types.
To isolate memory performance from pretrained knowledge,
Letta employs fictional question-answering datasets with artificially generated supporting facts.

$\infty$Bench 
~\citep{DBLP:journals/corr/abs-2402-13718}
distinguishes itself through unprecedented scale,
being the first benchmark with average context lengths exceeding 100K tokens.
The bilingual (English/Chinese) benchmark combines synthetic and realistic tasks
designed to require deep understanding of long-range dependencies,
where simple passage retrieval proves insufficient for successful completion.

\subsection{Comprehensive capabilities}
Although existing benchmarks primarily assess long-term memory through static or retrieval-based tasks, StoryBench 
~\citep{NEURIPS2023_f63f5fbe}
introduces a dynamic evaluation paradigm focused on interactive narrative reasoning.
Diverging from synthetic tests (e.g., Needle-in-a-Haystack) or conventional dialogue evaluations,
StoryBench simulates real-world memory demands through branching storylines where decisions propagate consequences.
The benchmark's innovative framework comprises 311 interconnected scenes with 86 decision points,
testing both knowledge retention (turn-to-turn coherence) and sequential reasoning (causal decision tracking).
StoryBench further innovates through dual evaluation modes:
Immediate feedback (assessing short-term error correction) and
self-recovery (evaluating autonomous mistake revision capabilities).

Minerva 
~\citep{xia2025minervaprogrammablememorytest}
contributes a unique programmable framework for decomposing memory capabilities into fundamental operations.
Unlike holistic benchmarks, Minerva enables precise examination of core memory functions through:
Atomic tests evaluating isolated skills (search, recall, edit, and stateful processing), and
composite tests simulating real-world scenarios through task combinations.
This modular approach facilitates the targeted analysis of specific memory subsystems and their interactions.


==> section/conclusion.tex <==
\section{Challenges and future directions}
As memory-augmented systems continue to evolve, several challenges remain unresolved, and addressing them will define the trajectory of future research. While progress has been notable in enhancing representational capacity, efficiency, and applicability, we present the following directions for future development:

\textbf{Towards Multimodal Memory}
Most existing memory models primarily focus on unimodal signals, making them less effective in real-world settings where information is inherently multimodal. Integrating visual, textual, and auditory information into a unified memory representation remains a fundamental challenge. Current research mainly applies the method of reducing multimodal information to text, which is simple yet inaccurate. A key difficulty lies in designing memory architectures that can not only store but also seamlessly align and retrieve information across different modalities. Furthermore, cross-modal reasoning requires mechanisms for resolving conflicts and ensuring consistency when modalities provide partially conflicting or redundant information. Future research directions include developing memory modules that fully exploit the potential of multimodal information.

\textbf{Towards Organized Memory}
Despite advances in increasing the capacity and retention length of memory models, most current approaches lack explicit organizational structures that resemble how humans categorize, cluster, and store knowledge. Without such organization, retrieval often depends heavily on similarity search, which can lead to inefficiencies or spurious outputs. A major research challenge is to design memory frameworks that can both self-organize and adapt their structures over time, facilitating more reliable inference and generalization. Promising directions involve hierarchical memory indexing, graph-based memory organization, and neuro-symbolic hybrids that combine distributed representations with explicit knowledge structuring. Such approaches may help models go beyond raw memorization, enabling reasoning patterns that remain stable over longer sequences and across tasks.

\textbf{Towards Multi-User Memory}
Another emerging challenge lies in extending memory systems to multi-user scenarios, where multiple agents or individuals interact with and contribute to a shared memory space. Unlike single-user settings, multi-user environments require mechanisms for managing overlapping, conflicting, or contradictory information while maintaining personalization. A critical dimension of this problem is privacy: memory modules must safeguard sensitive or user-specific data while still allowing useful knowledge to be shared and leveraged by others. Synchronization across different users introduces added complexity, as what one agent learns may be partially relevant, irrelevant, or even confidential for another. Addressing privacy requires fine-grained access control, anonymization protocols, and secure storage methods to prevent data leakage.

\section{Conclusion}
The growing body of research on memory in large language models reflects a decisive move toward systems capable of extending their knowledge, maintaining consistency, and reasoning across long timescales. Our survey has highlighted the complementary roles of external memory solutions—which emphasize interpretability and modular adaptability—and internal mechanisms—which focus on efficiency and tight integration within model architectures. Benchmarking efforts reveal that while significant progress has been made, current models still struggle with sustained recall, multimodal reasoning, and complex, real-world workflows. Several enduring challenges remain, such as developing richer organizational structures, ensuring scalability without excessive computational cost, and safeguarding privacy in shared or multi-user environments. Looking ahead, advances are likely to hinge on unifying multimodal signals, adopting hierarchical and graph-based structuring, and embedding trust, transparency, and security into memory systems. By addressing these directions, future research can enable LLMs to transition from reactive generators to adaptive, memory-empowered agents capable of supporting long-term human-AI collaboration.
























==> section/declarations.tex <==

\section*{Declarations}
\subsection*{Funding}
Not Applicable.

\subsection*{Conflicts of interest/Competing interests}
The authors declare that they have no known competing financial interests or personal relationships that could have appeared to influence the work in this manuscript.

\subsection*{Data availability}
All data used in this manuscript is publicly available. No new data was used for the research described in the manuscript.

\subsection*{Code availability}
The codes of baseline methods are from the public website.

\subsection*{Authors' contributions}

\subsection*{Acknowledgments}
We would like to thank the researchers in the field of training-free long video understanding for their foundational work. We are also grateful to the creators of the open-source benchmarks, which have greatly supported our research.

==> section/external_memory.tex <==
External memory mechanisms constitute one of the most prominent strategies for extending the recall and adaptability of LLMs. Unlike internal memory, which modifies or utilizes weights and intermediate states, external memory resides outside the model’s parameters, allowing updates and retrieval without costly retraining. By organizing past interactions or knowledge into interpretable formats such as text, graphs, or specialized databases, external memory systems provide transparency, flexibility, and persistent continuity. This section reviews key categories of external memory—text-based approaches, graph representations, and customized databases—highlighting how each constructs, manages, and retrieves information to enhance long-range reasoning and contextual consistency.

\subsection{Text}
Text-based memory systems form the foundation of most external memory approaches, distilling raw interactions and multimodal streams into natural language representations. By summarizing dialogue histories, creating event logs, or converting multimodal content into textual descriptions, these systems abstract rich interactions into compact and interpretable forms. The strength of text-based memory lies in its versatility: it can serve as a consistent record for dialogue systems, a bridge for multimodal integration, or the basis for downstream retrieval-augmented generation (RAG). In what follows, we discuss how text memory is constructed and subsequently retrieved to support LLM-based reasoning.

\subsubsection{Memory Construction}
The construction of text-based memory focuses on transforming past interactions into structured and persistent representations. Techniques range from simple conversation summaries to layered event hierarchies and biologically inspired encoding pipelines. By capturing user personas, episodic events, or multimodal inputs in textual form, these frameworks create a repository that can be directly queried or retrieved when needed. 

COMEDY~\citep{chen2024compressimpressunleashingpotential} proposes a compressive, text-native memory by converting each past session into session-level textual memories (natural-language summaries of events and user-bot attributes), then compressing the entire episode’s memories into a single, structured compressive memory text containing user profile, user–bot relationship dynamics, and a concise record of salient past events.
In MemoryBank~\citep{zhong2023memorybankenhancinglargelanguage}, each dialogue is first ingested as timestamped raw turns, which are periodically distilled by an LLM into daily event summaries and daily personality insights; these are further consolidated into global event summaries and a global user portrait, yielding a hierarchy: raw logs to daily summaries then global portrait.


% retreival
\subsubsection{Memory Retrieval}
Following the construction of the memory system, it is utilized to assist generation.
User input is first transformed into an embedding representation, which is then compared against a pre-indexed knowledge store using similarity search methods like dense vector retrieval or approximate nearest neighbor algorithms~\citep{lewis2021retrievalaugmentedgenerationknowledgeintensivenlp}. The top-ranked documents are returned to the model and concatenated with the original query, forming an enriched prompt that informs the generation process. 

Various search methods are introduced to find relevant memory.
Sparse retrieval techniques such as BM25~\citep{10.1561/1500000019} rely on keyword matching and term frequency–inverse document frequency (TF-IDF) weighting to identify passages with overlapping lexical features, offering efficiency and interpretability. Dense retrieval methods~\citep{karpukhin2020densepassageretrievalopendomain} employ neural embeddings trained on large corpora to capture semantic similarity beyond surface-level word overlap, often providing stronger recall in open-domain tasks. 
Hybrid approaches~\citep{gao2021rethinktrainingbertrerankers} combine sparse and dense retrieval to balance precision and coverage, while re-ranking models are applied to refine the initial candidate set before generation. Additionally, structured query methods, such as SQL-based search~\citep{liu2025surveytexttosqlerallms}, are leveraged in domains where relational databases dominate, allowing deterministic filtering and aggregation that complement vector-based retrieval. Together, these diverse retrieval strategies enhance the adaptability of RAG systems across heterogeneous data environments, ensuring that the generative model receives the most contextually relevant and accurate information for downstream tasks.

\subsubsection{Memory System}

Customized database along with its unique maintenance strategies are introduced in several memory frameworks to further ensure quality of the memory system.

Mem0~\citep{chhikara2025mem0buildingproductionreadyai} constructs memory incrementally from conversational interactions, representing knowledge as concise natural language facts. Its architecture employs a two-phase pipeline: during extraction, an LLM processes the latest message pair in conjunction with a conversation summary and a recency window to identify salient candidate facts; during update, these candidates are compared against existing memories from a vector database, and the model determines whether to add, update, delete, or ignore them. This ensures consistency and prevents redundancy. Retrieval is carried out through embedding-based similarity search, enabling the system to provide relevant memories as context for answering queries. In its graph-enhanced variant, Mem0$^g$, memories are represented as nodes and relations within a labeled knowledge graph, maintained through conflict detection and resolved updates, and retrieved via entity-centric or triplet-based queries for complex relational reasoning.

MemOS~\citep{li2025memosmemoryosai} treats memory as a first-class system resource, encapsulated in standardized units called MemCubes. Each MemCube contains both semantic payloads and metadata such as timestamp, provenance, and access permissions, supporting structured lifecycle management. Memory is categorized into three types: plaintext memory (explicit facts and documents), activation memory (short-term inference states such as KV-caches), and parameter memory (long-term encoded knowledge). Maintenance is governed by dedicated modules—MemScheduler, MemOperator, and MemLifecycle—that handle creation, activation, merging, and archiving, while also enabling cross-type migration such as distilling plaintext into parameter memory. Retrieval combines symbolic filtering and semantic embedding search, with MemScheduler dynamically selecting and injecting the most appropriate memory tier based on task intent, recency, and contextual relevance. This architecture allows MemOS to unify heterogeneous knowledge sources while supporting continual adaptation and traceable governance.

MIRIX~\citep{wang2025mirixmultiagentmemoryllmbased} organizes memory into six specialized components: Core, Episodic, Semantic, Procedural, Resource, and Knowledge Vault. Each component has a structured schema—for example, episodic memory stores events with summaries, details, and timestamps, while semantic memory encodes entities and concepts with definitions and descriptions. Maintenance is distributed across a multi-agent system, where each memory type has a dedicated manager and a Meta Memory Manager coordinates routing and updates. An active retrieval mechanism ensures that before answering a query, the agent generates a topical focus, which guides selective updating or rewriting of memory to avoid redundancy. Retrieval uses multiple strategies—embedding similarity, BM25 ranking, and string matching—depending on the query type. Retrieved items are labeled by memory category and incorporated into the system prompt, enabling coherent reasoning across personal facts, temporal sequences, procedural instructions, and sensitive data.

Letta (MemGPT)~\citep{packer2024memgptllmsoperatingsystems} adopts an operating system–inspired architecture, distinguishing between main context (system instructions, working context, and FIFO queue) and external context (recall and archival storage). Memory is formed by writing important conversational details or system events into the working context or recall storage, while overflow is managed by eviction policies that summarize older content and move it into archival storage. Maintenance is self-directed: the LLM issues function calls to add, update, or retrieve information, while the queue manager monitors capacity, generates recursive summaries, and enforces memory pressure warnings. Retrieval is achieved through paging, where relevant information is searched in recall or archival storage and reinserted into the active context window. By chaining multiple function calls, the system can iteratively recover long-range information, enabling LLMs to maintain consistent personas in dialogue and to analyze documents that exceed their native context length.

Across these frameworks, a clear divergence emerges in how memory is conceptualized, structured, and operationalized. Mem0 emphasizes efficiency and simplicity by encoding memories as concise natural language facts, with its graph-based extension  introducing relational richness to support more complex reasoning. MemOS, in contrast, takes a systems-level perspective, formalizing memory as a schedulable resource through MemCubes and lifecycle governance, allowing seamless transitions between explicit, activation, and parametric memories. MIRIX adopts a modular, multi-agent design, distributing responsibilities across specialized managers to capture different types of knowledge, with Active Retrieval ensuring task-oriented precision in both updating and querying. Finally, Letta (MemGPT) focuses on virtual context management, borrowing from operating system principles to create the illusion of infinite context through hierarchical paging between main and external memory tiers. Collectively, these approaches highlight a spectrum of strategies—from lightweight fact extraction to full-fledged operating system abstractions—demonstrating that the future of LLM memory systems will likely combine compact representations, structured graphs, lifecycle governance, and OS-style scheduling to achieve scalable, coherent, and contextually persistent intelligence.

\subsection{Graph}
Graph-structured memory approaches extend the representational capability of text summarization by embedding knowledge into nodes and edges. LLMs enhanced with graph memory benefit from both semantic interpretability and structural navigation, making them particularly effective for domains that demand persistent, interconnected knowledge. This section introduces graph-based memory along two primary dimensions: knowledge graph construction and hierarchical organizational frameworks.

\subsubsection{Knowledge Graph}
A knowledge graph (KG) is a structured representation of information that organizes entities—such as people, places, organizations, or events—and the relationships among them in the form of interconnected nodes and edges. Unlike traditional databases that rely on rigid tabular structures, knowledge graphs emphasize semantic connections, making them particularly powerful for reasoning, inference, and knowledge discovery~\citep{Hogan_2021}. The development of KGs stems from the need to transform unstructured or semi-structured data into formats that can be more easily queried and integrated across diverse domains. Early implementations, such as Google’s Knowledge Graph launched in 2012, popularized the concept by enhancing search engines with context-aware information retrieval~\citep{singhal2012knowledgegraph}. In academic research, KGs have gained prominence as a versatile tool for natural language processing (NLP), information extraction, and artificial intelligence applications, where they are often constructed through Knowledge Graph Construction (KGC) methods~\citep{Ji_2022}.

Several recent efforts in long-term memory for large language models converge on the use of knowledge graphs (KGs) as structured memory stores, where unstructured text is transformed into triples for retrieval and reasoning. HippoRAG~\citep{gutiérrez2025hipporagneurobiologicallyinspiredlongterm} draws inspiration from the hippocampal indexing theory, employing an LLM to perform open information extraction (OpenIE) over passages, turning them into schemaless triples of noun phrases and relations; synonym edges are then added through dense retrievers to link semantically similar phrases, and Personalized PageRank (PPR) is used at query time to traverse the KG for multi-hop retrieval. Building upon this, HippoRAG 2 ~\citep{gutiérrez2025ragmemorynonparametriccontinual} refines the process by integrating both phrase-level triples and full passages into the KG, treating phrases as sparse conceptual nodes and passages as dense contextual nodes, while also incorporating a recognition-memory step where an LLM filters retrieved triples to retain only relevant ones before PPR-based retrieval. In parallel, RET-LLM~\citep{modarressi2024retllmgeneralreadwritememory} also leverages OpenIE but explicitly encodes knowledge into triples of the form ⟨concept, relation, concept⟩ inspired by Davidsonian semantics, storing each in a memory table augmented with vector representations to support both exact and fuzzy retrieval. Similarly, Path Pooling~\citep{wang2025pathpoolingtrainingfreestructure} enhances triple-based KG-RAG by smoothing over paths: initial triples are retrieved via semantic scorers, then path kernels are searched using graph algorithms such as Dijkstra’s, and scores are pooled along these paths to incorporate structural signals into triple ranking without additional training. Knowledge Graph Tuning (KGT)~\citep{sun2024knowledgegraphtuningrealtime} extracts personalized factual triples from user interactions and directly edits the KG through additions and deletions, optimizing retrieval and reasoning probabilities without altering LLM parameters, thereby maintaining interpretability. Collectively, these methods illustrate a growing paradigm where LLM memory is externalized into explicit, interpretable triple-based KGs, enabling efficient updates, structural reasoning, and multi-hop retrieval beyond the limitations of pure vector storage.

Once stored as triples, these knowledge graphs are retrieved and utilized through a variety of mechanisms that aim to emulate the associative and contextual recall of human memory. HippoRAG~\citep{gutiérrez2025hipporagneurobiologicallyinspiredlongterm} retrieves information by first extracting named entities from a query using an LLM, linking them to corresponding KG nodes via dense embeddings, and then applying Personalized PageRank (PPR) to propagate probability mass across the graph, effectively enabling multi-hop retrieval in a single step; the resulting activated subgraph is then aggregated back into ranked passages for question answering. HippoRAG 2~\citep{gutiérrez2025ragmemorynonparametriccontinual} extends this process by allowing queries to be matched not only to nodes but also directly to triples, thereby preserving more contextual alignment, and introduces a recognition memory stage where an LLM filters out irrelevant triples before the PPR search, ensuring that only semantically coherent paths contribute to retrieval. Path Pooling~\citep{wang2025pathpoolingtrainingfreestructure} uses a different approach by first retrieving triples with a semantic scorer, then conducting graph searches to identify local path kernels, and finally smoothing scores across these paths via average pooling and positional weighting, which refines triple ranking for downstream generation. Knowledge Graph Tuning~\citep{sun2024knowledgegraphtuningrealtime} relies on the LLM to approximate the posterior distribution over relevant triples given a query and user feedback, optimizing the KG so that retrieval of personalized triples becomes more probable; during interaction, the LLM conditions its generation on the retrieved personalized triples, ensuring that responses reflect user-specific knowledge. Across these methods, retrieval is thus not limited to simple vector matching but leverages structural graph traversal, probabilistic weighting, and LLM-guided filtering, enabling richer multi-hop reasoning and adaptive, interpretable utilization of stored knowledge.

\subsubsection{Hierarchical Structures}
More graphs have been introduced to fully exploit the potential of memory system.
Zep~\citep{rasmussen2025zeptemporalknowledgegraph} introduces a temporally-aware dynamic knowledge graph, Graphiti, containing three hierarchical subgraphs: community subgraph - semantic entity subgraph - episode subgraph, which integrates episodic subgraphs storing raw conversations, semantic subgraphs encoding entities and their relationships, and community subgraphs capturing higher-level clusters, thereby enabling both temporal reasoning and efficient retrieval across long-term interactions. 
MIRIX~\citep{wang2025mirixmultiagentmemoryllmbased} routes user data into six specialized memory types, with semantic and episodic memories internally organized in hierarchical structures; here, graph-like organization emerges in semantic and procedural memories, where entities, concepts, and workflows are structured for efficient retrieval and abstraction.
AriGraph~\citep{anokhin2025arigraphlearningknowledgegraph} explicitly unifies semantic and episodic memory into a knowledge graph world model, where semantic triplets extracted from observations form vertices and edges, while episodic vertices store raw experiences connected through episodic edges linking co-occurring triplets, allowing the agent to maintain both factual structure and contextual temporal grounding.

Graph-based memory system features unique retrieval methods. Zep~\citep{rasmussen2025zeptemporalknowledgegraph} integrates cosine similarity, BM25 full-text search, and breadth-first search (BFS). BFS, a graph-specific retrieval technique, explores local neighborhoods within a configurable number of hops, facilitating the retrieval of contextually related entities and edges that may not be directly connected to the query. This enhances the discovery of relevance across structured relationships. Beyond BFS, hybrid search method is introduced in semantic and episodic memory integration~\citep{anokhin2025arigraphlearningknowledgegraph} within a hybrid graph model. Its semantic search employs a pre-trained contriever model to identify the most relevant triplets, while recursive graph traversal retrieves additional connected edges and nodes based on semantic similarity. GraphRAG~\citep{edge2025localglobalgraphrag} employs a dynamic label propagation algorithm for community detection, allowing retrieval by clustering related entities and edges into higher-level summaries. Hyperedge traversal, used in GraphReader~\citep{li2024graphreaderbuildinggraphbasedagent}, captures multi-entity relationships, enabling retrieval of complex facts that span several nodes. Distill-SynthKG~\citep{choubey2024distillsynthkgdistillingknowledgegraph} further enhances retrieval by combining subgraph expansion with key-value matching, ensuring the system retrieves both immediate and inferred knowledge. 


\subsection{Multi-modal}

Multi-RAG~\citep{mao2025multiragmultimodalretrievalaugmentedgeneration} forms text-first memories by converting all modalities to language: sampled frames are captioned with a VLM (with frame filtering to remove redundancies in low-change scenes), audio is transcribed with ASR, and auxiliary layers add temporal summaries and high-level analyses to preserve narrative flow. These timestamped texts are formatted (e.g., Markdown), chunked, and stored with pointers to the original media, yielding a layered, purely textual episodic record.

HippoMM~\citep{lin2025hippommhippocampalinspiredmultimodalmemory} builds memories through biologically inspired stages: it adaptively segments continuous streams into short events based on perceptual changes, encodes each event into a short-term memory with visual captions, speech transcripts, and cross-modal features, and then consolidates by removing redundant segments. A semantic replay step uses an LLM to produce concise, timestamped gist summaries linked back to detailed short-term content, forming compact long-term episodic text memories.


VideoAgent~\citep{wang2024videoagentlongformvideounderstanding} forms text memories by first captioning a small, uniformly sampled set of frames to establish an initial textual sketch of the video, then iteratively retrieving additional frames and converting them to captions as needed. An LLM orchestrates this loop: it assesses whether current captions suffice, specifies what visual evidence is missing and in which temporal segments to search, uses CLIP to fetch candidate frames, and invokes a VLM to translate those frames into concise textual descriptions. The growing, timestamped caption set—ordered and concatenated across rounds—constitutes the evolving text memory of the long video.




%\subsection{Others} Memvid https://github.com/Olow304/memvid turns millions of text chunks into a single, searchable video file by encoding text as QR codes in video frames, featuring 50 to 100 times smaller storage.

==> section/internal_memory.tex <==
While external memory mechanisms extend the capacity of language models to access and store information beyond their fixed parameters, internal memory plays an equally crucial role by optimizing how models handle information during inference. Internal memory mechanisms such as the parameter space and the key-value (KV) cache determine how efficiently models can process long contexts, balance computational costs, and preserve coherence across extended sequences. This section discusses the two major components of internal memory—KV-cache and parameters—along with strategies for managing, compressing, and constructing memory representations.

\subsection{KV-cache}
The KV-cache is a central element of transformer-based language models, enabling efficient reuse of intermediate attention representations across tokens. By storing key-value pairs from past tokens, the cache reduces redundant computation and allows models to handle longer sequences without recalculating attention states. However, maintaining and scaling the KV-cache introduces challenges in memory consumption, prompting research into better construction and management techniques.

\subsubsection{Construction}
The construction of the KV-cache involves how entries are initialized, updated, and integrated during inference. Research explores whether caches should store raw attention states or compressed abstractions, and how hierarchical or segment-level caching could improve scalability.

The standard Transformer builds the KV cache by saving all attention keys and values from each decoding step, leading to memory growth linear in sequence length and batch size. To mitigate this, methods such as Transformer-XL~\citep{dai2019transformerxlattentivelanguagemodels} introduce recurrence by caching past segment representations for reuse in subsequent segments, while Memorizing Transformer (MemTRM)~\citep{wu2022memorizingtransformers} extends this with external non-differentiable memory to store and retrieve KV pairs. 
More recent approaches like LongMem~\citep{wang2023augmentinglanguagemodelslongterm} decouple memory construction by using a frozen backbone LLM to encode past inputs into KV pairs, which are stored in a cache bank and later retrieved by a residual SideNet to avoid staleness. 
MA-LLM~\citep{He_2024_CVPR} integrates a long-term memory bank that auto-regressively accumulates visual and query embeddings, compresses redundant information, and feeds compact KV representations into the querying transformer for multimodal long-video understanding.
Memory³~\citep{Hongkang_Yang_2024} proposes explicit memory as a third storage format, where selected KV features are sparsified and stored externally, enabling retrieval akin to parameter-efficient caching. 
 redefines KV cache construction through selective retention, identifying “heavy-hitter” tokens via accumulated attention scores and maintaining only these along with the most recent tokens, thereby reducing memory by up to 5–10× while preserving accuracy. Together, these methods highlight a progression from dense caching to selective, compressed, and task-adaptive KV memory, aiming to balance efficiency, scalability, and performance in long-context LLMs.

\subsubsection{Management}
Management of the KV-cache focuses on balancing efficiency and scalability. Since the cache grows linearly with input length, naive use can quickly overwhelm GPU memory. Methods for selective retention, eviction, and compression are therefore critical for making long-context processing feasible.

Compression techniques aim to reduce the size of KV-cache representations while preserving essential context information. 
Traditional methods, such as H$_2$O~\citep{zhang2023h2oheavyhitteroracleefficient} and 
SnapKV~\citep{NEURIPS2024_28ab4182}, evaluate token importance through attention scores and dynamically prune less relevant tokens to reduce the cache size, albeit often at the expense of semantic coherence. 
Improvements like PyramidKV~\citep{cai2025pyramidkvdynamickvcache} and PyramidInfer~\citep{yang2024pyramidinferpyramidkvcache} leverage hierarchical patterns in attention scores, compressing KV caches layer-by-layer to minimize information loss. However, these token-level approaches often neglect semantic relationships between tokens, resulting in fragmented context. 
To address this, ChunkKV~\citep{liu2025chunkkvsemanticpreservingkvcache} introduces chunk-based compression, treating semantically meaningful groups of tokens as indivisible units, thus preserving linguistic structures while incorporating a layer-wise index reuse technique to enhance computational throughput. Additionally, methods such as ~\citet{xiao2024efficientstreaminglanguagemodels} and FastGen~\citep{ge2024modeltellsdiscardadaptive} focus on retaining the most recent or initial tokens, exploiting their higher attention scores across layers, while MiniCache~\citep{NEURIPS2024_fd070571} merges KV caches across layers to further reduce memory requirements. 

Beyond compression, active management strategies dictate which tokens or segments should remain in the cache.
PagedAttention~\citep{kwon2023efficientmemorymanagementlarge} tackles the inefficiency of contiguous allocation by partitioning the KV cache into fixed-size blocks, enabling near-zero memory waste and flexible sharing across beams or parallel samples. MemServe~\citep{hu2024memservecontextcachingdisaggregated} generalizes this idea by introducing MemPool, an elastic memory pool that abstracts KV cache placement and transfer across instances, supporting both inter-request techniques like context caching and intra-request methods such as disaggregated inference or sequence parallelism, while also incorporating global prompt-tree–based scheduling for cache reuse.
Infinite-LLM~\citep{lin2024infinitellmefficientllmservice} proposes DistAttention, which disaggregates attention computation by slicing KV cache along the sequence dimension and distributing it across multiple GPUs; through a mathematical reformulation, it minimizes communication overhead by shipping only lightweight query statistics instead of full KV tensors, thereby enabling cluster-level scheduling of sub-blocks of KV cache to balance computation and memory utilization. Together, these approaches demonstrate a shift from static, request-local cache allocations to dynamic, distributed, and fine-grained KV cache management strategies that improve throughput, reduce latency, and extend support to extremely long contexts in LLM serving.

\subsection{Parameters}
Parameter-based memory in LLMs focuses on directly encoding and updating knowledge within model weights, where different approaches vary in how they inject, adapt, or restructure parameters to serve as memory.

Early model editing methods such as ROME~\citep{meng2023locatingeditingfactualassociations} and MEMIT~\citep{meng2023masseditingmemorytransformer} treat feed-forward layers, particularly their value matrices, as key-value stores and directly overwrite weights to encode new factual associations. LoRA~\citep{hu2021loralowrankadaptationlarge} achieves parameter-efficient adaptation by freezing the pretrained weights and injecting trainable low-rank matrices alongside them, enabling lightweight updates without full fine-tuning.
Retrieval-augmented generation can be integrated into LoRA~\citep{10.1145/3721146.3721951}, treating adapters as hierarchical, modular memory units that can be incrementally trained, offloaded, and compacted, akin to log-structured merge trees. 
MEMORYLLM~\citep{wang2024memoryllmselfupdatablelargelanguage} further extends this idea by embedding a fixed-size memory pool of trainable hidden vectors within each transformer layer, which is continuously updated to absorb new knowledge while maintaining exponential forgetting dynamics.
WISE~\citep{wang2024wiserethinkingknowledgememory} introduces a dual parametric memory design with a “side memory” that receives edits while the main memory preserves pretrained knowledge, combined with sharding and merging mechanisms to ensure reliability, generalization, and locality in lifelong editing.

==> section/introduction.tex <==
The rapid advancement of large language models (LLMs) has fundamentally reshaped natural language processing (NLP) and artificial intelligence (AI) at large. With scaling laws demonstrating that increased model size and data lead to dramatic improvements in reasoning, comprehension, and generation~\citep{brown2020languagemodelsfewshotlearners},~\citep{touvron2023llamaopenefficientfoundation}, LLMs such as GPT, PaLM, and LLaMA have become the cornerstone of applications ranging from conversational agents to scientific discovery. Despite their impressive fluency and generalization, however, conventional LLMs remain constrained by their fixed context windows and static parameterization, which hinder their ability to maintain continuity, adapt over extended interactions, and accumulate knowledge across tasks~\citep{bubeck2023sparksartificialgeneralintelligence},~\citep{karpukhin2020densepassageretrievalopendomain}. These limitations have sparked a growing interest in augmenting LLMs with memory mechanisms.

Introducing memory into LLMs empowers them to transcend their stateless design and approximate more human-like cognition. By storing, retrieving, and adapting information across time, memory-augmented LLMs can sustain multi-session conversations, preserve user-specific knowledge, and execute complex workflows that require long-horizon reasoning~\citep{zhong2023memorybankenhancinglargelanguage},~\citep{chen2024compressimpressunleashingpotential}. Beyond dialogue, memory enables persistent adaptation in domains such as personal assistants, software engineering, education, and healthcare, where contextual consistency and long-term recall are critical~\citep{gutiérrez2025hipporagneurobiologicallyinspiredlongterm},~\citep{wang2025odysseybenchevaluatingllmagents} . Research has pursued both external memory architectures—such as text-based stores, knowledge graphs, and specialized databases—and internal memory mechanisms—such as parameter editing and efficient key-value (KV) caching~\citep{wu2022memorizingtransformers},~\citep{meng2023locatingeditingfactualassociations}. Together, these approaches mark a paradigm shift: from models that merely process text to systems capable of continual learning, temporal reasoning, and dynamic knowledge management.

This paper provides a comprehensive survey of recent progress on memory for LLMs. We review external memory approaches that construct and retrieve information through textual summaries, graphs, and structured databases, as well as internal memory strategies that optimize model parameters and KV-cache management. In addition, we examine benchmarks that have been proposed to evaluate memory capabilities, spanning both text-only and multimodal domains. We further highlight open challenges—including scalability, consistency, interpretability, and integration—and outline potential directions for future research. By synthesizing these developments, our contributions are threefold:
(1) We present a systematic taxonomy of memory mechanisms in LLMs, distinguishing between external and internal paradigms.
(2) We analyze representative frameworks, highlighting their design principles, retrieval strategies, and application scenarios.
(3) We review benchmark datasets and evaluation protocols, providing insights into how memory is currently measured and where progress is needed.

The remainder of this paper is structured as follows. Section 2 provides a broad overview of LLM memory research. Section 3 discusses external memory systems, including text-based, graph-based, and customized database approaches. Section 4 focuses on internal memory mechanisms, such as KV-cache construction and parameter adaptation. Section 5 surveys benchmarks for assessing memory capabilities. Section 6 outlines current challenges and future directions, while Section 7 concludes with a summary of key takeaways.


==> section/text_legacy.tex <==

\subsection{Memory Formation}
Memory can be extracted from the multi-turn conversations. 
To turn raw data into dataset suitable for long-term storage, various methodologies are adopted.




InfLLM~\citep{xiao2024infllmtrainingfreelongcontextextrapolation}
% https://arxiv.org/pdf/2402.04617
stores distant contexts into additional memory units.

LangMem
% https://github.com/langchain-ai/langmem
features two types of representation of memory: collections, to record an unbounded amount of knowledge to be searched at runtime,
and profiles, to record task-specific information that follows a strict schema that is easily looked up by user or agent.
Also, memories are divided into three categories: semantic for facts and knowledge,
episodic for past experiences, procedural for system behavior.

MIRIX~\citep{wang2025mirixmultiagentmemoryllmbased}
% https://arxiv.org/abs/2507.07957
further divides memory into six components,
including core memory for user information and preferences and knowledge vault for critical verbatim information.

MemOS~\citep{li2025memosmemoryosai}
% https://arxiv.org/abs/2507.03724
introduces MemCube to encapsulate all types of memory: parameter memory (model weights), activation memory (KV-cache), and plaintext memory (retrieved documents, prompts), for tracking, versioning, and governance.

MemoryBank~\citep{zhong2023memorybankenhancinglargelanguage}
% https://arxiv.org/pdf/2305.10250
generates a module to store
histories and their summaries, and maintains user profile.

Memvid
% https://github.com/Olow304/memvid
turns millions of text chunks into a single, searchable video file by encoding text as QR codes in video frames, featuring 50 to 100 times smaller storage.


% Parameter-wise
MemoryLLM~\citep{wang2024memoryllmselfupdatablelargelanguage}
% https://arxiv.org/abs/2402.04624
comprises a transformer and a fixed-size memory pool within the latent space of the transformer.
Self-updatable parameters are introduced to enable the model to integrate new knowledge.
queries

\subsection{Memory Management}

RMM (Reflective Memory Management)~\citep{tan2025prospectretrospectreflectivememory}
% https://arxiv.org/abs/2503.08026
integrates forward- and backward-looking reflections.
Prospective reflection dynamically summarizes interactions into a personalized memory bank
for effective future retrieval, and retrospective reflection iteratively refines retrieval
in an online reinforcement learning manner based on cited evidence from LLM.

MemoryBank~\citep{zhong2023memorybankenhancinglargelanguage}
% https://arxiv.org/pdf/2305.10250
incorporates a unique memory updating mechanism that mimics human-like memory behavior,
inspired by the Ebbinghaus Forgetting Curve theory.
This enables the AI to selectively forget or reinforce memories based on their significance and the passage of time.

A-Mem~\citep{xu2025amemagenticmemoryllm}
% https://arxiv.org/pdf/2502.12110
generates a comprehensive note containing multiple structured attributes during the formation, including contextual descriptions, keywords, and tags.
The system then analyzes historical memories to identify relevant connections, establishing links where there are meaningful similarities. 
As new memories are integrated, they can trigger updates to the contextual representations
and attributes of existing historical memories, allowing the memory network to continuously refine its understanding.

Zep~\citep{rasmussen2025zeptemporalknowledgegraph}
% https://arxiv.org/abs/2501.13956
builds a network of interconnected fact, each of which is a triplet represented by two entities (nodes) and their relationship (edge),
synthesizing both unstructured conversational data and structured business data while maintaining historical relationships.

MemoryOS~\citep{kang2025memoryosaiagent}
% https://arxiv.org/abs/2506.06326
enables dynamic updates among short-term, mid-term, and long-term personal memory:
short-term to mid-term updates following a dialogue-chain-based FIFO principle and
mid-term to long-term updates using a segmented page organization strategy.



\subsection{Retrieval Algorithm}
% https://aclanthology.org/2025.naacl-long.272.pdf


ChatDB~\citep{hu2023chatdbaugmentingllmsdatabases}
% https://arxiv.org/pdf/2306.03901
executes a series of intermediate memory operation steps to interact with symbolic memory.
ChatDB manipulates the symbolic memory in sequence according to a series of previously generated SQL statements,
including operations such as insert, update, select, delete, etc. The external database executes the corresponding SQL
statements, updates the database, and returns the results.

RET-LLM~\citep{modarressi2024retllmgeneralreadwritememory}
% https://arxiv.org/pdf/2305.14322
retrieves knowledge by converting user queries into structured triplet-based memory calls. 
The controller passes the query to the LLM, 
then the memory module first searches for exact matches in its triplet table and, 
if none are found, performs fuzzy retrieval using vector embeddings with locality-sensitive hashing. 
The retrieved triplets are then returned to the LLM, which generates a natural language answer for the user.

MemLLM~\citep{modarressi2025memllmfinetuningllmsuse}
% https://arxiv.org/pdf/2404.11672
adopts finetuning to train the model to access the explicit memory component through read
and write APIs to the memory module.

\subsection{Framework}
MemOS~\citep{li2025memosmemoryosai}
% https://arxiv.org/abs/2507.03724
features a three-layer architecture: interface layer, which translate user inputs or system prompts into structured memory,
operation layer which handles the organization, scheduling, transformation, and activation of memory resources during inference,
and infrastructure layer, which supports persistent storage, access control, governance, 
and synchronization of memory across users, tasks, and platforms. 

MIRIX~\citep{wang2025mirixmultiagentmemoryllmbased}
% https://arxiv.org/abs/2507.07957
employs a modular multi-agent workflow in which a central Meta Memory Manager coordinates 
with specialized Memory Managers to handle user interactions, 
memory updates, and information retrieval across six distinct memory components. 
When a user provides new input, the system automatically searches the memory base 
and forwards both the retrieved information and the input to the Meta Memory Manager, 
which determines the relevant memory types and routes the content to their respective managers 
for parallel updates, while avoiding redundancy. In conversational settings, 
the Chat Agent manages dialogue by initiating a broad memory search to gather high-level summaries, 
then refining retrieval through targeted queries to specific memory components using appropriate retrieval strategies. 
It consolidates the results into coherent responses, while also applying updates when users introduce new facts or corrections, 
thereby ensuring that responses remain accurate, contextually grounded, and dynamically aligned with evolving knowledge.


Letta~\citep{packer2024memgptllmsoperatingsystems}
% https://arxiv.org/abs/2310.08560
has an OS-inspired hierarchical memory with virtual context management
, which can intelligently handle different storage tiers in order to effectively provide extended context 
within limited context window.
Letta is able to analyze large documents and multi-session chat that far exceed the window,
where it can create conversational agents that remember, reflect, and evolve dynamically 
through long-term interactions with their users.


mem0~\citep{chhikara2025mem0buildingproductionreadyai}
% https://arxiv.org/abs/2504.19413
applies a two-phase memory pipeline that extracts, consolidates, and retrieves only the most salient conversational facts: 
In the extraction phase, the system ingests three context sources—the latest exchange, 
a rolling summary, and the m most recent messages—and uses an LLM to extract a concise set of candidate memories. 
A background module refreshes the long-term summary asynchronously, so inference never stalls.
In the update phase, each new fact is compared to the similar entries in the vector database. 
The LLM then chooses one of four operations: add, update, delete or no operation.


